Unbalanced Random Matching Markets with Partial Preferences

Properties of stable matchings in the popular random-matching-market model have been studied for over 50 years. In a random matching market, each agent has complete preferences drawn uniformly and independently at random. Wilson (1972), Knuth (1976) and Pittel (1989) proved that in balanced random matching markets, the proposers are matched to their $\ln n$th choice on average. In this paper, we consider markets where agents have partial (truncated) preferences, that is, the proposers only rank their top $d$ partners. Despite the long history of the problem, the following fundamental question remained unanswered: \emph{what is the smallest value of $d$ that results in a perfect stable matching with high probability?} In this paper, we answer this question exactly -- we prove that a degree of $\ln^2 n$ is necessary and sufficient. That is, we show that if $d < (1-\epsilon) \ln^2 n$ then no stable matching is perfect and if $d > (1+ \epsilon) \ln^2 n$, then every stable matching is perfect with high probability. This settles a recent conjecture by Kanoria, Min and Qian (2021). We generalize this threshold for unbalanced markets: we consider a matching market with $n$ agents on the shorter side and $n(\alpha+1)$ agents on the longer side. We show that for markets with $\alpha =o(1)$, the sharp threshold characterizing the existence of perfect stable matching occurs when $d$ is $\ln n \cdot \ln \left(\frac{1 + \alpha}{\alpha + (1/n(\alpha+1))} \right)$. Finally, we extend the line of work studying the effect of imbalance on the expected rank of the proposers (termed the ``stark effect of competition''). We establish the regime in unbalanced markets that forces this stark effect to take shape in markets with partial preferences.

==> game.tex <==
\section{Preliminaries}

\subsection{A probability game}
\label{sec:game}

Define a multi-round probabilistic game as follows. In each round, there are three events that can occur: $G$ (Good), $B$ (Bad), and $N$ (Neutral).  Given an input parameter $d$,  for each round, conditioned on the events in previous rounds, define
$\Pr(G) = p_G$, $\Pr(B) \geq p_B$ and $\Pr(N) = p_N$.  The game is \defn{won} if $G$ occurs.  The game is \defn{lost} if $B$ occurs $d$ times in a row.  Then we have the following bound on the probability of winning this game, denoted by $\Pr_{\text{win}}(p_G, p_B)$.

\begin{theorem}


\begin{equation*}
  \Pr_{\text{\em win}}(p_G, p_B) \leq \frac{p_G (1-p_B)}{p_G + p_N \cdot (p_B)^d} \leq \frac{p_G}{p_B^d}
\end{equation*}
\end{theorem}

\begin{proof}
Suppose the game is played for $i$ rounds, and let $S = (s_1, s_2, \ldots, s_i)$ denote the random sequence of events that occur.  Consider a new game that is the same as the original except now $\Pr(B) = p_B$, and let $S' = (s_1', s_2', \ldots, s_i')$ denote the random sequence of events that occur in this game.  
%
Let $\Pr_{\text{win}'}$ be the winning probability in the new game.  Through a coupling argument, we show that 
$\Pr_{\text{win}} \leq \Pr_{\text{win}'}$.

Given the sequence $S'$, we create a sequence $S$ as follows:  for $i\geq 0$, as long as the game does not end in a loss at $i$ rounds, do:
\begin{itemize}
    \item if $s_i' = G$, then $s_i = G$,
    \item if $s_i' = B$, then $s_i = B$,
    \item if $s_i' = N$, then $s_i = N$ with probability $\frac{1 - p_G - p_B^i}{1 - p_G - p_B}$ and $s_i = B$ otherwise.  
    Here $p_B^i = \Pr(s_i = B~|~ s_{i-1}, \ldots, s_1) \geq p_B$.  
\end{itemize}
Note that whenever $S'$ ends in a loss (event $B$ occurs $d$ times in a row), then $S$ also ends in a loss.   Thus, $\Pr_{\text{win}} \leq \Pr_{\text{win}'}$.  

Finally, we show that $\Pr_{\text{win}'} = \frac{p_G (1-p_B)}{p_G + p_N \cdot (p_B)^d}$ through the following recurrence.

\begin{align*}
\Pr_{\text{win}'} &= p_G + p_N \cdot \Pr_{\text{win}'} + p_B \cdot p_N \cdot \Pr_{\text{win}'} + p_B^2 \cdot p_N \cdot \Pr_{\text{win}'}  + \ldots +  p_B^{d-1} \cdot p_N \cdot \Pr_{\text{win}'}\\
&= p_G + p_N \cdot \Pr_{\text{win}'} (1  + p_B + p_B^2 + \ldots + p_B^{d-1})\\
&= p_G + p_N \cdot \Pr_{\text{win}'} \left( \frac{1- p_B^d}{1-p_B}\right)\\
\Pr_{\text{win}'} &= \frac{p_G(1-p_B)}{1 - p_B - p_N + p_N \cdot p_B^d}\\
 &= \frac{p_G(1-p_B)}{p_G + p_N \cdot p_B^d}\\
 & = \frac{p_G(p_G+p_N)}{p_G + p_N\cdot p_B^d}\\
 & \leq \frac{p_G}{p_B^d}\qedhere
\end{align*}

\end{proof}

\begin{proposition}\label{prop:unmatchedwomen}
Consider a random matching market with $n$ women and competitive factor $\alpha$, where $m = n (\alpha + 1)$. In a men-proposing deferred acceptance algorithm (MPDA), we have that after $\tau$ proposals have been made, for any $\gamma > 0$ the number of unmatched women $\delta^w (\tau)$:

\begin{align*}
 \mathbb{P}(\delta^w(\tau) &> (1 + \gamma)ne^{-\frac{\tau}{n}}) \leq \frac{2e^{\tau/n}}{\gamma^2n}\\
  \mathbb{P}(\delta^w(\tau) &< (1 - \gamma)ne^{-\frac{\tau}{n}}) \leq \frac{2e^{\tau/n}}{\gamma^2n}
\end{align*} 


\end{proposition}


